Demonstration of Safe Electromagnetic Radiation Emitted by 5G Active Antenna Systems

The careful planning and safe deployment of 5G technologies will bring enormous benefits to society and the economy. Higher frequency, beamforming, and small-cells are key technologies that will provide unmatched throughput and seamless connectivity to 5G users. Superficial knowledge of these technologies has raised concerns among the general public about the harmful effects of radiation. Several standardization bodies are active to put limits on the emissions which are based on a defined set of radiation measurement methodologies. However, due to the peculiarity of 5G such as dynamicity of the beams, network densification, Time Division Duplexing mode of operation, etc, using existing EMF measurement methods may provide inaccurate results. In this context, we discuss our experimental studies aimed towards the measurement of radiation caused by beam-based transmissions from a 5G base station equipped with an Active Antenna System(AAS). We elaborate on the shortcomings of current measurement methodologies and address several open questions. Next, we demonstrate that using user-specific downlink beamforming, not only better performance is achieved compared to non-beamformed downlink, but also the radiation in the vicinity of the intended user is significantly decreased. Further, we show that under weak reception conditions, an uplink transmission can cause significantly high radiation in the vicinity of the user equipment. We believe that our work will help in clearing several misleading concepts about the 5G EMF radiation effects. We conclude the work by providing guidelines to improve the methodology of EMF measurement by considering the spatiotemporal dynamicity of the 5G transmission.

==> 7-acknowledgement.tex <==
%The authors would like to thank the Fraunhofer IIS OAI team for implementing the OAI software customization for NTNs. In addition, we would like to thank the OAI Software Alliance for developing the 5G OSS ecosystem. Special gratitude goes to the Bundeswehr Cyber and Information Domain Service for providing satellite capacity. The views expressed herein can in no way be taken to reflect the official opinion of the European Space Agency.
This work is supported by the Luxembourg Government -Department of Media, Telecommunications and Digital Policy-for the Project ref SMC/CFP-II/03, SAFER (Demonstration of SAFE electromagnetic Radiation emitted by 5G active antennas systems

%The authors would like to acknowledge the projects SAFER (Demonstration of SAFE electromagnetic Radiation emitted by 5G active antennas systems) and IRANATA (Interference and RAdiation in Network PlAnning of 5G AcTive Antenna Systems) both funded by the \textit{Service des Médias et des Communications} (SMC) of the Government of the Grand Duchy of Luxembourg.

==> X-5g-nr-emf-concerns-and-measurement-challenges.tex <==
\begin{comment}
	\item Here we first discuss what are the features in 5G-NR which are creating the concern. Make figures. Use thr table which shows difference between 4g and 5g from emf point of view. 
	\item Next we will discuss the emf measurement challenged in 5G-NR but before that we will briefly discuss the three measurement tech and count their pros and cons.  
\end{comment}

Although 5G-NR still uses OFDM for uplink and downlink, it has gone through significant changes on Radio Access Network (RAN); especially the way in which the waveforms are transmitted from the gNB. Besides, different frequency bands (FR1 and FR2), wider bandwidths (100MHz for FR1 and 400 MHz for FR2) and Time Division Duplexing are some of the peculiarities in 5G which are in contrast to the RAN of 4G LTE. Discussion on such difference between 4G and 5G is important from EMF radiation point of view. In this section, first we focus on the specific features in 5G-NR which are creating concern among general public. Next we point out some of the challenges while performing EMF measurement in the 5G network. 

%5G will initially operate in conjunction with existing 4G networks (either in NSA, i.e., Non-Stand-Alone mode or co-existence mode) before evolving to fully Stand Alone (SA) networks in subsequent releases\cite{liu20205g}. 3GPP has defined two different frequency ranges for 5G: FR1(4.1GHz to 7.125GHz and maximum bandwidth of 100MHz) which is attractive for coverage reasons and FR2(24.25GHz to 52.6GHz), also known as millimeter waves and capable of providing extremly high bandwidth upto 400MHz, though at the cost of reduced coverage. Both FDD and TDD modes of duplexing are supported, however, TDD dominates the current deployment. On the physical layer 5G-NR uses Orthogonal Frequency Division Multiple Access (OFDM-A) in the downlink and uplink, however, the SubCarrierSpacing (SCS) is not fixed in 5G, it is flexible. The SCS scales by $ 2\mu \times15 $ kHz to cover different frequency ranges and service (QoS and latency) requirements\cite{zaidi2016waveform,arslan2018flexible}. 

\begin{comment}[h]
	\centering
	\includegraphics[width=\linewidth]{nr-ssb-frame}
	\caption{5G-NR SSB frame structure}
	\label{fig:nr-ssb-frame}
\end{comment}
\begin{comment}[h]
	\centering
	\includegraphics[width=\linewidth]{beamformed-pbch-pdsch-pdcch}
	\caption{}
	\label{fig:beamformed-pbch-pdsch-pdcch}
\end{comment}
\begin{comment}[h]
	\centering
	\includegraphics[width=\linewidth]{extrapolation-factors9}
	\caption{}
	\label{fig:extrapolation-factors9}
\end{comment}
\begin{comment}[h]
	\centering
	\includegraphics[width=\linewidth]{beamformed-pbch-pdsch-pdcch1}
	\caption{a good question is how long the ssb is visible}
	\label{fig:beamformed-pbch-pdsch-pdcch1}
\end{comment}
\begin{comment}[h]
	\centering
	\includegraphics[width=\linewidth]{emf-meas-with-ssb}
	\caption{SSB suits all the criterion for code selective beamforming}
	\label{fig:emf-meas-with-ssb}
\end{comment}
\begin{comment}[h]
	\centering
	\includegraphics[width=\linewidth]{extrapolation-factors8}
	\caption{}
	\label{fig:extrapolation-factors8}
\end{comment}
%\subsubsection{Beamformed PBCH, PDCCH and PDSCH}
%Regulations typically require that the highest possible power and gain values are used when calculating the RF EMF exposure to ensure conservative results. 

%5G NR uses beamforming to overcome the path loss for synchronization (SSBs) and data signals. It is an essential method to overcome the increasing path loss when using higher frequencies. AAS is used for this purpose which create very narrow but high-gain beams to focus the power on a certain area to increase SINR and received power.

%In contrast to LTE, where sectoral antennas which make wide beams were used for the broadcast of PBCH, 5G-NR uses so-called Synchronization Signal Blocks (SSB) bursts which are narrower in beam width, the process is called beamforming. 

\subsection{Massive MIMO}\label{sub-massive-mimo}
Massive MIMO is one of the most important 5G technologies. It contains a large number of antenna elements, typically on the base-station side. Through digital and/or analog control of the RF chains, one or many user-centric sharp beams can be created and the beams can be further adapted dynamically based on the user movement and requirements [\textbf{REF}]. A controller is required for such operation which can be either colocated with the antenna units or through RF cables. The former one constitutes an Active Antenna System which has became the dominate configuration in the ongoing deployment of 5G base-stations. 

Superfically, one can one can correspond large number of antenna elements to increased amount of radiated power which in turn can strengthen the myth about higher radiation from 5G base-station. In fact, the maximum transmitted power by a 5G BS can reach up to 200 W, almost double the corresponding value for a 4G BS\cite{elzanaty20215g}. This increase in power triggers the population’s concern about potential health risks. However, this is not the fact. A Massive MIMO system aims to project focused power towards user locations and in this process, compared to a sectoral-antenna Less power per-antenna-element is required in order to achieve the \textit{same SNR} a sectoral-antenna would have provided[\textbf{REF}]. This happens because the antenna array can concentrate the input energy in the desired direction and minimizes the radiation in the undesired direction, thus less input energy is required per antenna element.

\subsection{Beamformed Channels and Signals}
5G, inherently uses beamforming using AAS as discussed in section-\ref{sub-massive-mimo}. Not only the user-centric data(payload and control) is beamformed, but the synchronization signals, which are used to set-up the time-frequency alignment are also transmitted as beams. The former is called user-specific beamforming and is done for PDSCH and PDCCH while the later is called Synchronization Signal Blocks (SSBs) beam-sweeping which is done for PSS, SSS and PBCH. User specific beams could be sharper than the beams used for SSBs. Besides, the beams can be parsed in both azimuth and elevation with the application of an AAS. 

Such beam based operations are also one of the cause of public concerns regarding radiation from 5G base-station. A crude perception of beam, among general public is seen as focussed beam of energy towards them, and hence beams are seen as a cause of concern. However, the reality is different. For a desired SNR at the intended user, the transmit power from a sectoral antenna is higher compared to an antenna array with high gain and directivity. Besides, the radiation from the sectoral antenna not only reaches to the intended user but also gets spreaded in the vicinity unnecessarily. In contrast, the antenna array elements inside the AAS, require less input power per antenna element for a given target SNR at the intended user and at the same time minimize the splill of radiation in the vicinity of the intended user.   

%Moreover, AAS is capable of managing the beam dynamically. This is very different from traditional network planning where sector-level wide beams were used which were also static in nature. 5G uses such beam based approach for not only the data and control channels (PDSCH and PDCCH) but also for the synchronization signals (PBCH in SSB). 5G uses bursts of synchronization signals called SSB burst [\textbf{REF}] which sweeps both azimuth and elevation. This process is called beam-sweeping. 

%\subsubsection*{Massive MIMO and Beamforming--MERGE}


%However, there are two substantial differences compared to previous networks, i.e., higher maximum output power and dynamic pencil beamforming with a larger number of antenna elements. The maximum transmitted power by a 5G BS can reach up to 200 W, almost double the corresponding value for a 4G BS\cite{elzanaty20215g}. This increase in power can trigger the population’s concern about potential health risks.


%5G NR uses beamforming to overcome the path loss for synchronization (SSBs) and data signals. For that purpose, Active Antenna Arrays create very narrow but high-gain beams to focus the power on a certain area for increasing the SINR and received power. Such operation crates field strength hotspots in the very narrow main lobes of the beams. The adoption of these new technological features has resulted in heightened concerns about exposure health effects.

%Although the maximum radiated power in 5G is higher than that of 4G, the radiation intensity is 25\% of the maximum exposure for 95\% of the cases. -- I need to get some result like this. 

%It aims to project power to user locations, thereby improving coverage and reducing inter-cell interference. 
%5G static broadcast beams cover the entire cell using the narrow-beam polling mode. 

\subsection{mmWave and network densification}
Millimeter-wave (mmWave) frequency bands contain large signal bandwidth and are very promising for 5G to reach data rate as high as 10 Gb/s. Mm-Wave provides a much larger bandwidth, higher throughput, faster data rate, and capacity compared with, 3G, 4G. Hence, 5G networks are planned to be deployed in FR2 (for higher bandwidth use-cases) apart from FR1 ( more favourable for coverage). However, the benefits of mmWave comes at the cost of reduced coverage. mmWave cannot travel as far as the frequencies used in 2G/3G/4G. To cope-up with this, either beamforming is done on the mmWave carrier (discussed in section-\ref{sub-massive-mimo}) and/or the base-stations have to be placed densly. The later is called network desnsification and this has raised concern among the general public concerning radiation. 

However, at the same time, the implementation of mmWave new technologies has increased the population concern over the possible impact on health and safety arising from the radiated electromagnetic field (EMF) exposure by these systems. 

%Millimeter waves (MMWs) are mostly absorbed within 1 to 2 millimeters of human skin and in the surface layers of the cornea \cite{moskowitz}.  
%FIRST TELL WHY MMWAVE IS NOT INHERENTLY HARMFUL THEN THE FOLLOWING ARGUMENT. 
%High node density. 
%However, the benefits of mmWave comes at a cost of reduced coverage. mmWave cannot travel as far as the frequencies used in 4G can travel. There are two solutions for this:
\begin{comment}
	\item Network densification 
	\item Beamforming (directional transmission)
\end{comment}

%5G NR uses beamforming to overcome the path loss for synchronization (SSBs) and data signals. 

%higher frequencies are now combined with beamforming 

\subsection{Network Densification}
Small cells. 

Smallcells: less power required to macro cells  but but but 

In order to support an increasing number of users with higher data rates, installing additional BSs over the territory is essential, i.e., network densification. Therefore, the distance between the users and the nearest cell shrinks, increasing the perceived health impacts.

Unlike the common opinion, network densification can significantly reduce the average EMF exposure for a given required rate (Chiaraviglio et al., 2020a; Chiaraviglio et al., 2019). In fact, the cell coverage area is smaller for networks with higher BS density, requiring lower transmitted power. On the contrary, networks with fewer BSs exhibit a larger coverage area and a higher radiated power for each cell. Furthermore, dense networks are endowed with a homogeneous distribution of power over the territory; hence, the EMF exposure is distributed more uniformly among the population. For networks with smaller densities, users close to BSs are exposed to higher radiation than those at the edge. In other words, network densification reduces both the average and the variance of the exposure over the area compared to legacy networks (Chiaraviglio et al., 2020a, Chiaraviglio et al., 2020d).

Besides extremely fast wireless data speeds, the next generation mobile technology will require many more towers than previously needed to provide wireless services due to use of sub 6 GHz and mmWave frequencies. To provide reliable connections, this dense network of 5G towers will be located in neighborhoods rather than distant remote locations, where the large majority of wireless towers are currently located.

The concern with having so many towers based so close to humans is the high-frequency millimetersized radio waves that 5G uses to deliver extremely fast data will increase human exposure to EMFs. This calls for a timely evolution of EMF exposure assessment methodology for 5G.

\subsection{High Uplink Traffic}
Traffic patterns are changing. More uplink heavy applications are anticipated (e.g. cloud storage and personal broadcasting) and flexibility with uplink and downlink spectrum usage has already been foreseen. That is why TDD has become the dominant deployment mode in 5G. TDD uses the same frequency for each duplex direction, with a frame that includes different time periods and slots for uplink or downlink communications. By changing the duration of these, network performance can be tailored to meet different needs and help provide the best possible experience. A rise of such uplink traffic is a genuine concern from the EMF point of view, especially when the RSSI at the UE is poor. Due to power control 

Such high uplink traffic raises concern especially when the 5G UE is near to the user and the RSSI of the UE is poor. 

\begin{comment}
\begin{table}[t]
\caption{ Main differences between 5G and predecessor 4G technologies}
\label{tab:1}
\centering
\small
\begin{tabular}{|p{2cm}|p{2.5cm}|p{2.5cm}|}
\hline
\textbf{Feature } & \textbf{4G}& \textbf{5G}\\
\hline
Antenna pattern & Fixed, same for signaling and data & Beam forming\\
\hline
Beam pattern  & Azimuth: $60^\circ$or$360^\circ$ Elevation:$\sim 10^\circ$ & Depending on type of signal and
antenna\\
\hline
Frequency range  &  $400$ MHz to $6$ GHz  & FR1: $400$ MHz to $7$ GHz.
FR2: 28 GHz, 38 GHz, (43, 47,
beyond)
\\
\hline
RF bandwidth & $\leq 20$ MHz & $\leq 100$ MHz (FR1), $\leq  400$ MHz (FR2)\\
\hline
Signaling & In mid of frequency band, always on,
same pattern as data & At fixed frequencies, not necessarily in
same band, beam constant or scanning\\
\hline
\end{tabular}
\end{table}
\end{comment}




==> related-work.tex <==


\begin{itemize}
	\item Review of EMF radiation methodology for 5G base stations with Active Antenna Systems
	\item No standardized protocol and existing is deprecated 
	\item Extrapolations accounting temporal \& spatial variabilities
\end{itemize}


